Enhancing energy transport utilising permanent molecular dipoles

We study exciton quantum transfer along a molecular chain whilst accounting for the effects of permanent dipoles that are induced by charge displacements in the molecular orbitals. These effects are typically neglected as they do not arise in atomic quantum optics; however, they can play an important role in molecular systems. We also consider novel collective photon-assisted transport and compare it against the scaling of phonon-assisted transport in chains featuring permanent dipoles, and determine a linear scaling with the number of dipoles, akin to single-excitation superradiance. We further demonstrate how permanent dipoles, dipoles can preferentially arrange energy eigenstates to support excitation transport. Finally, we show how permanent dipoles can enhance the ability of the molecular chain to support excitation transport compared to that of systems that do not possess permanent dipoles across a range of environmental and system configurations.

==> derivations.tex <==
\begin{align}
    B^n_\text{vib} &= |\bra{\Psi_D} \sigma_z^{(n)} \ket{\Psi_B}|^2\nonumber\nonumber\\
    &= \left|\frac{1}{{N}}\sum_{j=1}^N\bra{j}(-1)^j \sigma_z^{(n)}\sum_m \ket{m}\right|^2\nonumber\\
    &=  \left|\frac{1}{{N}}\sum_{j=1}^N\bra{j}(-1)^j(2\delta_{nm}-1)\sum_m \ket{m}\right|^2\nonumber\\
    &= \left|\frac{1}{{N}}\sum_{j,m=1}^N(-1)^j(2\delta_{nm}-1) \delta_{jm}\right|^2\nonumber\\
    &= \left|\frac{1}{{N}}2(-1)^n\right|^2 = \frac{4}{N^2},
\end{align}

\begin{align}
    B_\text{opt} &= \left| \bra{\Psi_D}\sum_{n=1}^N \sigma_z^{(n)}\mathbf{d}_z^{(n)}\ket{\Psi_B}\right|^2\nonumber\\
    &= \left|\frac{1}{N}\sum_{j,k,n=1}^N\bra{j}(-1)^j\mathbf{d}_z^{(n)}(2\delta_{nk}-1)\ket{k} \right|^2\nonumber\\
    &=  \left|\frac{1}{N}(2\sum_{k=1}^N(-1)^k\mathbf{d}_z^{(k)} -\mathbf{d}_z^+(-1)^k \right|^2 \nonumber\\
    &= \left|\frac{1}{N}2\sum_{k=1}^N(-1)^k\mathbf{d}_z^{(k)}\right|^2\nonumber\\
    &= \frac{4}{N^2}\left|\sum_{k=1}^N(-1)^k\mathbf{d}_z^{(k)}\right|^2. 
\end{align}
